Probing the Excitation of Extreme Starbursts: High Resolution Mid-IR Spectroscopy of Blue Compact Dwarfs

We present an analysis of the mid-infrared emission lines for a sample of 12 low metallicity Blue Compact Dwarf (BCD) galaxies based on high resolution observations obtained with Infrared Spectrograph on board the {\rm Spitzer} Space Telescope. We compare our sample with a local sample of typical starburst galaxies and active galactic nuclei (AGNs), to study the ionization field of starbursts over a broad range of physical parameters and examine its difference from the one produced by AGN. The high-ionization line [OIV]25.89$\mu$m is detected in most of the BCDs, starbursts, and AGNs in our sample. We propose a diagnostic diagram of the line ratios [OIV]25.89$\mu$m/[SIII]33.48$\mu$m as a function of [NeIII]15.56$\mu$m/[NeII]12.81$\mu$m which can be useful in identifying the principal excitation mechanism in a galaxy. Galaxies in this diagram split naturally into two branches. Classic AGNs as well as starburst galaxies with an AGN component populate the upper branch, with stronger AGNs displaying higher [NeIII]/[NeII] ratios. BCDs and pure starbursts are located in the lower branch. We find that overall the placement of galaxies on this diagram correlates well with their corresponding locations in the log([NII]/H$\alpha$) vs. log([OIII]/H$\beta$) diagnostic diagram, which has been widely used in the optical. The two diagrams provide consistent classifications of the excitation mechanism in a galaxy. On the other hand, the diagram of [NeIII]15.56$\mu$m/[NeII]12.81$\mu$m vs. [SIV]10.51$\mu$m/[SIII]18.71$\mu$m is not as efficient in separating AGNs from BCDs and pure starbursts. (abridged)

==> authors <==
Probing the Excitation of Extreme Starbursts: High Resolution
Mid-IR Spectroscopy of Blue Compact Dwarfs

Lei Hao, Yanling Wu, V. Charmandaris, H. W. W. Spoon, J. Bernard-Salas, D. Devost, V. Lebouteiller, and J. R. Houck 

15 pages, including 1 table and 14 figures. Accepted by ApJ


We present an analysis of the mid-infrared emission lines for a sample
of 12 low metallicity Blue Compact Dwarf (BCD) galaxies based on high
resolution observations obtained with Infrared Spectrograph on board
  the {\rm Spitzer} Space Telescope. We compare our sample with a local
  sample of typical starburst galaxies and active galactic nuclei
  (AGNs), to study the ionization field of starbursts over a broad
  range of physical parameters and examine its difference from the one
  produced by AGN. The high-ionization line [OIV]25.89$\mu$m is
  detected in most of the BCDs, starbursts, and AGNs in our sample. We
  propose a diagnostic diagram of the line ratios
  [OIV]25.89$\mu$m/[SIII]33.48$\mu$m as a function of
  [NeIII]15.56$\mu$m/[NeII]12.81$\mu$m which can be useful in
  identifying the principal excitation mechanism in a galaxy. Galaxies
  in this diagram split naturally into two branches. Classic AGNs as
  well as starburst galaxies with an AGN component populate the upper
  branch, with stronger AGNs displaying higher [NeIII]/[NeII]
  ratios. BCDs and pure starbursts are located in the lower branch. We
  find that overall the placement of galaxies on this diagram
  correlates well with their corresponding locations in the
  log([NII]/H$\alpha$) vs. log([OIII]/H$\beta$) diagnostic diagram,
which has been widely used in the optical. The two diagrams provide
  consistent classifications of the excitation mechanism in a
  galaxy. On the other hand, the diagram of
  [NeIII]15.56$\mu$m/[NeII]12.81$\mu$m
  vs. [SIV]10.51$\mu$m/[SIII]18.71$\mu$m is not as efficient in
  separating AGNs from BCDs and pure starbursts.  Our analysis
  demonstrates that BCDs in general do display higher [NeIII]/[NeII]
  and [SIV]/[SIII] line ratios than starbursts, with some reaching
  values even higher than those found at the centers of AGNs. Despite
  their hard radiation field though, no [NeV]14.32$\mu$m emission has been
  detected in the BCDs of our sample.

